Spectroscopic Binary Orbits from Photoelectric Radial Velocities - Paper 191: HD 17310, HD 70645 and HD 80731

The three objects have been identified as members of the recently recognized class of Gamma Doradus stars, which exhibit multi-periodic photometric variations that are thought to arise from non-radial pulsation. The particular objects treated here also prove to be spectroscopic binaries, for which we provide reliable orbits. The radial velocities exhibit unusually large residuals, in which some of the photometric periodicities can be traced. Some of the same periodicities are also demonstrated by the observed variations in the line profiles, which are quantified here simply in terms of the line-widths.

==> p191t1.tex <==
\nopagenumbers
\hsize=11truecm          \vsize=25.0 true cm     
\hoffset=2.9truecm       \voffset0.0truecm
\baselineskip=12pt	 \overfullrule=0pt        \parindent0truecm
\font\rm=cmr10           \font\bf=cmbx10	  \font\math=cmsy10
\font\it=cmti10          \font\tt=cmtt10          \tolerance=250
\font\brm=cmr10 scaled\magstep1          \font\bit=cmti10 scaled\magstep1
\font\bbf=cmbx10 scaled\magstep2                  \font\ssrm=cmr10 at 6pt
\font\srm=cmr10 at 8pt   \font\sit=cmti10 at 8pt  \font\sbf=cmbx10 at 8pt
\font\smdag=cmsy10 at 8pt\font\ssit=cmti10 at 6pt 
\def\cl{\centerline}     \def\ni{\noindent}       \def\ii{\itemitem}
\def\bs{\bigskip}        \def\ms{\medskip}	  \def\ss{\smallskip}
\def\vs#1{\vskip#1pt}    \def\eqo{\eqalignno}     \parskip=0pt
\def\vfe{\vfill\eject}   \def\hf{\hfil}          \def\hah{\hfill & \hfill}
\def\hcr{\hfill & \cr}   \def\hrfa{\hrulefill &} \def\hrfb{\hfill & \hrulefill}
\def\nl{\hfil\break\ni}  \def\PM{\hs1 $\pm$ \hs1}
\def\np{\par\ni\hangindent=1.0 true cm\hangafter=1}
\def\up#1{\raise.8ex\hbox{\ssrm#1}}     \def\bsk#1{\baselineskip#1pt}
\def\sa{\rlap{$^{\ast}$}}               \def\"{\hs3\lower0.5ex\hbox{"}}
\def\sb{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'171}}}
\def\sc{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'172}}}
\def\sd{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'170}}}
\def\se{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'173}}}
\def\sf{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'153}}}
\def\sg{\rlap{\hs{0.4}$^{\ast\ast}$}}
\def\si{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'172\char'172}}}
\def\s#1{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm#1}}}
\def\sC{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm C}}}
\def\sG{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm G}}}
\def\sI{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm I}}}
\def\sN{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm N}}}
\def\sR{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm R}}}
\def\sT{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm T}}}
\def\sU{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm U}}}
\def\sW{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm W}}}
\def\ta{\llap{$^{\ast}$}\hs1}       
\def\tb{\llap{\raise.6ex\hbox{\smdag\char'171}}\hs1}
\def\tc{\llap{\raise.6ex\hbox{\smdag\char'172}}\hs1}
\def\td{\llap{\raise.6ex\hbox{\smdag\char'170}}\hs1}
\def\te{\llap{\raise.6ex\hbox{\smdag\char'173}}\hs1}
\def\tf{\llap{\raise.6ex\hbox{\smdag\char'153}}\hs1}
\def\tg{\llap{$^{\ast\ast}$}}
\def\ti{\llap{\raise.6ex\hbox{\smdag\char'172\char'172}}}
\def\t#1{\llap{\raise.7ex\hbox{\ssrm #1}}\hs0}
\def\tC{\llap{\raise.7ex\hbox{\ssrm C}}\hs1}
\def\tG{\llap{\raise.7ex\hbox{\ssrm G}}\hs1}
\def\tI{\llap{\raise.7ex\hbox{\ssrm I}}\hs1}
\def\tN{\llap{\raise.7ex\hbox{\ssrm N}}\hs1}
\def\tR{\llap{\raise.7ex\hbox{\ssrm R}}\hs1}
\def\tT{\llap{\raise.7ex\hbox{\ssrm T}}\hs1}
\def\tU{\llap{\raise.7ex\hbox{\ssrm U}}\hs1}
\def\tW{\llap{\raise.7ex\hbox{\ssrm W}}\hs1}
\def\thsp{\thinspace}    \def\msp{\kern.4em}     \def\sk{\hskip.6em\relax}
\def\kms{km~s$^{-1}$}    \def\kmss{km~s$^{-1}$\kern.25em}
\def\itkms{\hbox{{\it km s}\raise.6ex\hbox{\sit\hs{0.8}--\hs{0.5}1}}\hs1}
%\def\apjkms{\rm K{\srm M \hs1 S}$^{-1}$}
\def\asec{$''$}          \def\asecl{$''$\llap}   
\def\etal{{\it et al\/}.\hs3}       \def\setal{{\sit et al\/}.}
\def\etal#1{{\it et al\/}.\hs{-1.3}$^{#1}$}  
\def\b-v{($B-V$)}                   \def\u-b{($U-B$)}
\def\sec{\hbox{$''$\hskip-3pt .}}   \def\tsec{\hbox{$^s$\hskip-3pt .}}
\def\min{\hbox{$'$\hskip-3pt .}}    \def\tmin{\hbox{$^m$\hskip-3pt .}}
\def\Amm{\AA~mm$^{-1}$}             \def\Amms{\AA~mm$^{-1}$\kern .35em}
\def\msun{$M_{\odot}$\thsp}         \def\rsun{$R_{\odot}$\thsp}
\def\mbol{$M_{bol}$\thsp}           \def\mbs{$M_{bol \odot}$\thsp}
\def\degl{$^{\circ}$\hskip-1pt .}   \def\deg{\hbox{$^{\circ}$\hskip-3pt .}}
\def\dego{\raise.9ex\hbox{\smdag\char'16}}   \def\degs{\dego\hs3}
\def\hs#1{\hskip#1pt}               \def\hm#1{\hskip#1em} 
\def\frac#1/#2{\leavevmode\kern.05em\raise.6ex\hbox{\the\scriptfont0
    #1}\kern-.15em/\kern-.15em\lower.3ex\hbox{\the\scriptfont0 #2}}
\def\smfrac#1/#2{\leavevmode\kern.05em\raise.4ex\hbox{\the\scriptscriptfont0
    #1}\kern-.15em/\kern-.15em\lower.2ex\hbox{\the\scriptscriptfont0 #2}}
\def\itfrac#1/#2{\leavevmode\kern.05em\raise.6ex\hbox{\the\sit
    #1}\kern-.15em/\kern-.15em\lower.3ex\hbox{\the\sit #2}\hs1}
\def\itfracs#1/#2{\leavevmode\kern.05em\raise.6ex\hbox{\the\sit
    #1}\kern-.15em/\kern-.15em\lower.3ex\hbox{\the\sit #2}\hs4}
\def\corstop{\hbox{{\it C\hs{-1} oravel\/}.}\hs5}
\def\corcom{\hbox{{\it C\hs{-1} oravel\/},}\hs4}
\def\cor{\hbox{{\it C\hs{-1} oravel\/}}}      \def\cors{\cor\hs4}
\def\smcor{\hbox{\sit C\hs{-0.5}oravel\/}}    \def\smcors{\smcor\hs4}
\def\m{\hbox{\raise.8ex\hbox{\srm m}}}
\def\mag{\hbox{\raise.8ex\hbox{\srm m}\hskip-1pt .}}
\def\x{\hbox{\raise.2ex\hbox{,,}}}
\def\cont{(\hs{-1}{\it C\hs{-0.5}ontinued\/}\hs{0.5})}
\def\wt{wt.\hs{1.5}}


\hsize13truecm\hoffset1.4truecm
\tabskip1.9em \def\vsini{\hbox{`$v$\hs{1.5}sin\hs{1.5}$i$'}}
\brm\cl{\hm{-0.5}T{\rm ABLE} I}\ms\bit
\cl{\hm{-0.5}Radial-velocity observations    of HD 70645            }
\bs\it
\hm{3.2}Date \hm{0.2}{\rm (}\hs{-1}UT\/{\rm )}\it\hm{3.8}MJD\hm{2.2}Velocity
\hm{1.2}Phase\hm{1.6}{\rm (}$O-C${\rm )\hm{1.2}\it`\hs1v\hs{1.5}sin\hs{1.5}i'}\vs1\vs1
\hm{16.4}\itkms\hm{6.1}\itkms\hm{1.5}\itkms
\rm\halign{\hm{-0.5}#\hfil\hm{-2.0}&\hfil#&\hfil#&    \hfil$#$\hm{0.2}&
\hm{-0.5}\hfil#\hm{0.2}&\hfil$#$&\hm1#\hfil\cr
\noalign{\filbreak\vs{12}}
 2003\hs4Mar. &10.279\sa&  52708.279&  +44.4&$\overline{   116}$.887&   -2.3\cr
\hskip2em 
     \hs4Apr. &30.159\sa&    759.159&  +44.7&$\overline{   110}$.915&   +0.8\cr
\noalign{\filbreak\vs{12}}
 2004\hs4Sept.&26.505\sa&  53274.505&  +34.7&$\overline{    49}$.974&   +0.3\cr
\noalign{\filbreak\vs{12}}
 2005\hs4Nov. &14.178&  53688.178&  +31.2&     0.986&   -0.7&13\cr
\hskip2em 
     \hs4     &19.176&    693.176&  +17.5&     1.578&   +1.6&11.5\cr
\hskip2em 
     \hs4     &25.182&    699.182&  -18.4&     2.290&   -0.9&12\cr
\hskip2em 
     \hs4     &30.183&    704.183&  +45.6&.882&   -1.5&11.5\cr
\hskip2em 
     \hs4Dec. &15.131&    719.131&  +26.9&     4.653&   -2.4&12\cr
\hskip2em 
     \hs4     &17.172&    721.172&  +47.9&.895&   +1.9&12\cr
\hskip2em 
     \hs4     &18.119&    722.119&  +29.7&     5.007&   +2.5&12\cr
\noalign{\filbreak\vs{12}}
 2006\hs4Jan. &26.016&  53761.016&  +22.4&     9.616&   -0.3&13.5\cr
\hskip2em 
     \hs4Feb. &15.991&    781.991&   +3.7&    12.101&   -1.5&11\cr
\hskip2em 
     \hs4     &16.905&    782.905&  -12.6&.209&   +0.6&10.5\cr
\hskip2em 
     \hs4     &17.998&    783.998&  -15.9&.339&   +0.4&12\cr
\hskip2em 
     \hs4     &18.867&    784.867&   -7.7&.442&   -1.2&\hm{0.5}9.5\cr
\hskip2em 
     \hs4     &20.887&    786.887&  +35.4&.681&   +1.4&14\cr
\hskip2em 
     \hs4Mar. & 1.920&    795.920&  +41.1&    13.751&   -2.5&10.5\cr
\hskip2em 
     \hs4     & 4.927&    798.927&   +3.2&    14.108&   -0.5&16\cr
\hskip2em 
     \hs4     & 6.006&    800.006&  -18.6&.236&   -3.1&11.5\cr
\hskip2em 
     \hs4     & 6.909&    800.909&  -15.6&.343&   +0.5&14\cr
\hskip2em 
     \hs4     &24.918&    818.918&   -4.5&    16.476&   -3.0&11.5\cr
\hskip2em 
     \hs4Apr. & 3.994&    828.994&  +33.5&    17.670&   +1.4&12\cr
\hskip2em 
     \hs4     & 4.938&    829.938&  +44.0&.782&   -2.4&11\cr
\hskip2em 
     \hs4     & 6.057&    831.057&  +41.5&.915&   -2.5&\hm{0.5}7.5\cr
\hskip2em 
     \hs4     & 8.962&    833.962&  -16.3&    18.259&   +0.5&13.5\cr
\hskip2em 
     \hs4     &10.915&    835.915&   +3.5&.490&   +2.9&11.5\cr
\hskip2em 
     \hs4     &12.022&    837.022&  +21.4&.621&   -2.3&15.5\cr
\hskip2em 
     \hs4     &14.872&    839.872&  +37.9&.959&   +0.7&10\cr
\hskip2em 
     \hs4     &25.915&    850.915&  -17.6&    20.267&   -0.5&\hm{0.5}9.5\cr
\hskip2em 
     \hs4     &27.898&    852.898&   +1.1&.502&   -1.5&15.5\cr
\hskip2em 
     \hs4     &29.854&    854.854&  +42.7&.734&   +1.2&11.5\cr
\hskip2em 
     \hs4May  & 1.947&    856.947&  +31.5&.982&   -1.2&11\cr
\hskip2em 
     \hs4     & 2.974&    857.974&   +4.7&    21.104&   +0.1&10\cr
\hskip2em 
     \hs4     & 5.970&    860.970&   -6.1&.459&   -2.0&14\cr
\hskip2em 
     \hs4     & 9.866&    864.866&  +42.8&.920&   -0.5&12\cr
\hskip2em 
     \hs4     &10.892&    865.892&  +19.4&    22.042&   +0.3&12\cr
\hskip2em 
     \hs4     &11.901&    866.901&   -5.0&.161&   +1.6&14\cr
\hskip2em 
     \hs4     &15.928&    870.928&  +27.5&.638&   +0.8&11\cr
\hskip2em 
     \hs4     &16.868&    871.868&  +43.6&.750&   +0.2&12.5\cr
\hskip2em 
     \hs4     &18.876&    873.876&  +31.3&.988&   -0.2&11.5\cr
\hskip2em 
     \hs4     &21.885&    876.885&  -14.0&    23.344&   +2.0&13\cr
\hskip2em 
     \hs4     &23.886&    878.886&  +19.3&.581&   +2.9&13.5\cr
\hskip2em 
     \hs4     &29.893&    884.893&  -16.1&    24.293&   +1.4&10\cr
\hskip2em 
     \hs4     &30.896&    885.896&   -8.9&.412&   +1.3&11.5\cr
\hskip2em 
     \hs4     &31.896&    886.896&   +6.8&.530&   -0.6&15.5\cr
\hskip2em 
     \hs4June & 2.893&    888.893&  +47.6&.767&   +2.5&12\cr
\hskip2em 
     \hs4     & 3.893&    889.893&  +50.8&.885&   +4.0&13.5\cr
}
\vs{10}\parskip0pt
\cl{\hm3\ta Observation published by Henry {\it et al.}$^9$.}\par
\cl{\hm3 All others observed with the Cambridge \cor .}\par
\bye


==> p191t3.tex <==
\magnification950
\nopagenumbers
\hsize=11truecm          \vsize=25.0 true cm     
\hoffset=2.9truecm       \voffset0.0truecm
\baselineskip=12pt	 \overfullrule=0pt        \parindent0truecm
\font\rm=cmr10           \font\bf=cmbx10	  \font\math=cmsy10
\font\it=cmti10          \font\tt=cmtt10          \tolerance=250
\font\brm=cmr10 scaled\magstep1          \font\bit=cmti10 scaled\magstep1
\font\bbf=cmbx10 scaled\magstep2                  \font\ssrm=cmr10 at 6pt
\font\srm=cmr10 at 8pt   \font\sit=cmti10 at 8pt  \font\sbf=cmbx10 at 8pt
\font\smdag=cmsy10 at 8pt\font\ssit=cmti10 at 6pt 
\def\cl{\centerline}     \def\ni{\noindent}       \def\ii{\itemitem}
\def\bs{\bigskip}        \def\ms{\medskip}	  \def\ss{\smallskip}
\def\vs#1{\vskip#1pt}    \def\eqo{\eqalignno}     \parskip=0pt
\def\vfe{\vfill\eject}   \def\hf{\hfil}          \def\hah{\hfill & \hfill}
\def\hcr{\hfill & \cr}   \def\hrfa{\hrulefill &} \def\hrfb{\hfill & \hrulefill}
\def\nl{\hfil\break\ni}  \def\PM{\hs1 $\pm$ \hs1}
\def\np{\par\ni\hangindent=1.0 true cm\hangafter=1}
\def\up#1{\raise.8ex\hbox{\ssrm#1}}     \def\bsk#1{\baselineskip#1pt}
\def\sa{\rlap{$^{\ast}$}}               \def\"{\hs3\lower0.5ex\hbox{"}}
\def\sb{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'171}}}
\def\sc{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'172}}}
\def\sd{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'170}}}
\def\se{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'173}}}
\def\sf{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'153}}}
\def\sg{\rlap{\hs{0.4}$^{\ast\ast}$}}
\def\si{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'172\char'172}}}
\def\s#1{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm#1}}}
\def\sC{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm C}}}
\def\sG{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm G}}}
\def\sI{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm I}}}
\def\sN{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm N}}}
\def\sR{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm R}}}
\def\sT{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm T}}}
\def\sU{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm U}}}
\def\sW{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm W}}}
\def\ta{\llap{$^{\ast}$}\hs1}       
\def\tb{\llap{\raise.6ex\hbox{\smdag\char'171}}\hs1}
\def\tc{\llap{\raise.6ex\hbox{\smdag\char'172}}\hs1}
\def\td{\llap{\raise.6ex\hbox{\smdag\char'170}}\hs1}
\def\te{\llap{\raise.6ex\hbox{\smdag\char'173}}\hs1}
\def\tf{\llap{\raise.6ex\hbox{\smdag\char'153}}\hs1}
\def\tg{\llap{$^{\ast\ast}$}}
\def\ti{\llap{\raise.6ex\hbox{\smdag\char'172\char'172}}}
\def\t#1{\llap{\raise.7ex\hbox{\ssrm #1}}\hs0}
\def\tC{\llap{\raise.7ex\hbox{\ssrm C}}\hs1}
\def\tG{\llap{\raise.7ex\hbox{\ssrm G}}\hs1}
\def\tI{\llap{\raise.7ex\hbox{\ssrm I}}\hs1}
\def\tN{\llap{\raise.7ex\hbox{\ssrm N}}\hs1}
\def\tR{\llap{\raise.7ex\hbox{\ssrm R}}\hs1}
\def\tT{\llap{\raise.7ex\hbox{\ssrm T}}\hs1}
\def\tU{\llap{\raise.7ex\hbox{\ssrm U}}\hs1}
\def\tW{\llap{\raise.7ex\hbox{\ssrm W}}\hs1}
\def\thsp{\thinspace}    \def\msp{\kern.4em}     \def\sk{\hskip.6em\relax}
\def\kms{km~s$^{-1}$}    \def\kmss{km~s$^{-1}$\kern.25em}
\def\itkms{\hbox{{\it km s}\raise.6ex\hbox{\sit\hs{0.8}--\hs{0.5}1}}\hs1}
%\def\apjkms{\rm K{\srm M \hs1 S}$^{-1}$}
\def\asec{$''$}          \def\asecl{$''$\llap}   
\def\etal{{\it et al\/}.\hs3}       \def\setal{{\sit et al\/}.}
\def\etal#1{{\it et al\/}.\hs{-1.3}$^{#1}$}  
\def\b-v{($B-V$)}                   \def\u-b{($U-B$)}
\def\sec{\hbox{$''$\hskip-3pt .}}   \def\tsec{\hbox{$^s$\hskip-3pt .}}
\def\min{\hbox{$'$\hskip-3pt .}}    \def\tmin{\hbox{$^m$\hskip-3pt .}}
\def\Amm{\AA~mm$^{-1}$}             \def\Amms{\AA~mm$^{-1}$\kern .35em}
\def\msun{$M_{\odot}$\thsp}         \def\rsun{$R_{\odot}$\thsp}
\def\mbol{$M_{bol}$\thsp}           \def\mbs{$M_{bol \odot}$\thsp}
\def\degl{$^{\circ}$\hskip-1pt .}   \def\deg{\hbox{$^{\circ}$\hskip-3pt .}}
\def\dego{\raise.9ex\hbox{\smdag\char'16}}   \def\degs{\dego\hs3}
\def\hs#1{\hskip#1pt}               \def\hm#1{\hskip#1em} 
\def\frac#1/#2{\leavevmode\kern.05em\raise.6ex\hbox{\the\scriptfont0
    #1}\kern-.15em/\kern-.15em\lower.3ex\hbox{\the\scriptfont0 #2}}
\def\smfrac#1/#2{\leavevmode\kern.05em\raise.4ex\hbox{\the\scriptscriptfont0
    #1}\kern-.15em/\kern-.15em\lower.2ex\hbox{\the\scriptscriptfont0 #2}}
\def\itfrac#1/#2{\leavevmode\kern.05em\raise.6ex\hbox{\the\sit
    #1}\kern-.15em/\kern-.15em\lower.3ex\hbox{\the\sit #2}\hs1}
\def\itfracs#1/#2{\leavevmode\kern.05em\raise.6ex\hbox{\the\sit
    #1}\kern-.15em/\kern-.15em\lower.3ex\hbox{\the\sit #2}\hs4}
\def\corstop{\hbox{{\it C\hs{-1} oravel\/}.}\hs5}
\def\corcom{\hbox{{\it C\hs{-1} oravel\/},}\hs4}
\def\cor{\hbox{{\it C\hs{-1} oravel\/}}}      \def\cors{\cor\hs4}
\def\smcor{\hbox{\sit C\hs{-0.5}oravel\/}}    \def\smcors{\smcor\hs4}
\def\m{\hbox{\raise.8ex\hbox{\srm m}}}
\def\mag{\hbox{\raise.8ex\hbox{\srm m}\hskip-1pt .}}
\def\x{\hbox{\raise.2ex\hbox{,,}}}
\def\cont{(\hs{-1}{\it C\hs{-0.5}ontinued\/}\hs{0.5})}
\def\wt{wt.\hs{1.5}}


\hsize13truecm\hoffset2truecm\vsize27truecm\voffset-0.5truecm\bsk{11}
\tabskip1.9em \def\vsini{\hbox{`$v$\hs{1.5}sin\hs{1.5}$i$'}}
\brm\cl{\hm{-2.5}T{\rm ABLE} III}\ms\bit
\cl{\hm{-2.5}Radial-velocity observations    of HD 80731            }
\bs\it
\hm{3.2}Date \hm{0.2}{\rm (}\hs{-1}UT\/{\rm )}\it\hm{3.8}MJD\hm{2.2}Velocity
\hm{1.55}Phase\hm{1.3}{\rm (}$O-C${\rm )}\it\hm{1.2}`\hs1v\hs{1.5}sin\hs{1.5}i'\vs1
\hm{16.4}\itkms\hm{6.1}\itkms\hm{1.5}\itkms
\rm\halign{\hm{-0.5}#\hfil\hm{-2.0}&\hfil#&\hfil#&    \hfil$#$\hm{0.2}&
\hfil#\hm{0.2}&\hfil$#$&\hm1#\hfil\cr
\noalign{\filbreak\vs7}
 2003\hs4Mar. & 8.307\sa&  52706.307&   -8.7&$\overline{    93}$.987&   -1.1&\cr
\hskip2em 
     \hs4     & 9.283\sa&    707.283&  +17.2&$\overline{    92}$.079&   -0.8&\cr
\hskip2em 
     \hs4     &10.314\sa&    708.314&  +11.6&.175&   -9.0&\cr
\hskip2em 
     \hs4May  & 1.258\sa&    760.258&  +12.4&$\overline{    87}$.041&   +2.0&\cr
\noalign{\filbreak\vs7}
 2004\hs4Apr. &24.202\sa&  53119.202&   -9.2&$\overline{    54}$.668&   +2.3&\cr
\hskip2em 
     \hs4     &25.192\sa&    120.192&  -18.7&.761&   -0.4&\cr
\hskip2em 
     \hs4     &28.215\sa&    123.215&  +11.0&$\overline{    53}$.044&   -0.1&\cr
\noalign{\filbreak\vs7}
 2005\hs4Nov. &19.213&  53693.213&   +0.7&     0.443&   -3.4&15\cr
\hskip2em 
     \hs4     &25.191&    699.191&   -2.6&     1.003&   -0.4&16.5\cr
\hskip2em 
     \hs4     &30.193&    704.193&   +0.9&.471&   -1.3&14\cr
\hskip2em 
     \hs4Dec. &15.148&    719.148&  -24.8&     2.872&   -0.6&17.5\cr
\hskip2em 
     \hs4     &17.177&    721.177&  +15.9&     3.062&   +0.6&12\cr
\hskip2em 
     \hs4     &18.131&    722.131&  +17.7&.152&   -3.6&13.5\cr
\hskip2em 
     \hs4     &26.946&    730.946&  -11.8&.978&   -1.0&14.5\cr
\hskip2em 
     \hs4     &28.022&    732.022&  +19.3&     4.078&   +1.4&12\cr
\noalign{\filbreak\vs7}
 2006\hs4Jan. &26.007&  53761.007&  -20.3&     6.794&   +0.2&14.5\cr
\hskip2em 
     \hs4     &27.242&    762.242&  -22.5&.909&   +0.9&11.5\cr
\hskip2em 
     \hs4Feb. &15.997&    781.997&  -16.4&     8.760&   +1.8&14.5\cr
\hskip2em 
     \hs4     &16.919&    782.919&  -23.9&.847&   -0.4&18.5\cr
\hskip2em 
     \hs4     &18.009&    784.009&  -16.8&.949&   +1.6&19.5\cr
\hskip2em 
     \hs4     &18.876&    784.876&   +5.7&     9.030&   -1.4&14.5\cr
\hskip2em 
     \hs4     &20.896&    786.896&  +17.4&.219&   -1.2&10.5\cr
\hskip2em 
     \hs4Mar. & 1.035&    795.035&   -8.4&.982&   +1.1&13.5\cr
\hskip2em 
     \hs4     & 1.931&    795.931&  +15.8&    10.066&   -0.1&11.5\cr
\hskip2em 
     \hs4     & 3.042&    797.042&  +21.1&.170&   +0.3&14.5\cr
\hskip2em 
     \hs4     & 3.865&    797.865&  +17.1&.247&   +0.1&18\cr
\hskip2em 
     \hs4     & 4.936&    798.936&  +13.0&.347&   +2.5&16\cr
\hskip2em 
     \hs4     & 6.016&    800.016&   +5.4&.448&   +1.6&\hm{0.5}9.5\cr
\hskip2em 
     \hs4     & 6.917&    800.917&   +0.5&.533&   +2.5&14\cr
\hskip2em 
     \hs4     &22.921&    816.921&  +10.1&    12.032&   +2.4&15\cr
\hskip2em 
     \hs4Apr. & 4.002&    829.002&  +22.2&    13.164&   +1.2&13.5\cr
\hskip2em 
     \hs4     & 5.053&    830.053&  +17.6&.262&   +1.5&13.5\cr
\hskip2em 
     \hs4     & 6.068&    831.068&   +9.7&.357&   -0.2&15\cr
\hskip2em 
     \hs4     & 8.957&    833.957&   -9.6&.628&   -1.0&17\cr
\hskip2em 
     \hs4     &10.933&    835.933&  -23.8&.813&   -2.0&13\cr
\hskip2em 
     \hs4     &12.029&    837.029&  -23.5&.916&   -0.5&12\cr
\hskip2em 
     \hs4     &14.880&    839.880&  +21.7&    14.183&   +1.3&20\cr
\hskip2em 
     \hs4     &25.925&    850.925&  +19.7&    15.217&   +1.0&13\cr
\hskip2em 
     \hs4     &27.912&    852.912&   +6.5&.404&   -0.3&16\cr
\hskip2em 
     \hs4May  & 1.961&    856.961&  -19.9&.783&   -0.1&12\cr
\hskip2em 
     \hs4     & 2.964&    857.964&  -22.4&.877&   +1.9&15\cr
\hskip2em 
     \hs4     & 5.996&    860.996&  +21.9&    16.161&   +0.8&14\cr
\hskip2em 
     \hs4     & 9.901&    864.901&   -2.9&.527&   -1.3&\hm{0.5}9.5\cr
\hskip2em 
     \hs4     &10.915&    865.915&   -6.0&.622&   +2.2&13\cr
\hskip2em 
     \hs4     &11.915&    866.915&  -13.2&.715&   +1.8&12\cr
\hskip2em 
     \hs4     &15.941&    870.941&  +20.1&    17.093&   +0.6&21\cr
\hskip2em 
     \hs4     &16.969&    871.969&  +20.0&.189&   -0.1&18.5\cr
\hskip2em 
     \hs4     &18.915&    873.915&   +7.0&.371&   -1.9&13\cr
\hskip2em 
     \hs4     &21.913&    876.913&  -13.2&.652&   -2.9&15.5\cr
\hskip2em 
     \hs4     &26.943&    881.943&  +21.8&    18.123&   +0.6&14.5\cr
\hskip2em 
     \hs4     &29.921&    884.921&   +8.9&.402&   +2.0&16\cr
\hskip2em 
     \hs4     &30.929&    885.929&   +0.3&.497&   -0.2&17\cr
\hskip2em 
     \hs4     &31.908&    886.908&   -6.1&.588&   -0.3&16\cr
\hskip2em 
     \hs4June & 2.910&    888.910&  -19.4&.776&   -0.1&19\cr
\hskip2em 
     \hs4     & 3.917&    889.917&  -27.1&.870&   -2.9&23.5\cr
\hskip2em 
     \hs4     & 5.914&    891.914&  +10.2&    19.057&   -4.1&17\cr
\hskip2em 
     \hs4     & 8.925&    894.925&   +9.5&.340&   -1.6&12.5\cr
\hskip2em 
     \hs4     & 9.923&    895.923&   +2.9&.433&   -1.9&14.5\cr
\hskip2em 
     \hs4     &10.926&    896.926&   -1.8&.527&   -0.2&11\cr
\hskip2em 
     \hs4     &11.917&    897.917&   -7.4&.620&   +0.6&17\cr
\hskip2em 
     \hs4     &12.920&    898.920&  -14.3&.714&   +0.5&15\cr
}
\vs{10}\parskip0pt
\cl{\hm1\ta Observation published by Henry {\it et al.}$^9$.}\par
\cl{\hm1 All others observed with the Cambridge \cor .}\par
\bye


==> p191t5.tex <==
\nopagenumbers
\hsize=11truecm          \vsize=25.0 true cm     
\hoffset=2.9truecm       \voffset0.0truecm
\baselineskip=12pt	 \overfullrule=0pt        \parindent0truecm
\font\rm=cmr10           \font\bf=cmbx10	  \font\math=cmsy10
\font\it=cmti10          \font\tt=cmtt10          \tolerance=250
\font\brm=cmr10 scaled\magstep1          \font\bit=cmti10 scaled\magstep1
\font\bbf=cmbx10 scaled\magstep2                  \font\ssrm=cmr10 at 6pt
\font\srm=cmr10 at 8pt   \font\sit=cmti10 at 8pt  \font\sbf=cmbx10 at 8pt
\font\smdag=cmsy10 at 8pt\font\ssit=cmti10 at 6pt 
\def\cl{\centerline}     \def\ni{\noindent}       \def\ii{\itemitem}
\def\bs{\bigskip}        \def\ms{\medskip}	  \def\ss{\smallskip}
\def\vs#1{\vskip#1pt}    \def\eqo{\eqalignno}     \parskip=0pt
\def\vfe{\vfill\eject}   \def\hf{\hfil}          \def\hah{\hfill & \hfill}
\def\hcr{\hfill & \cr}   \def\hrfa{\hrulefill &} \def\hrfb{\hfill & \hrulefill}
\def\nl{\hfil\break\ni}  \def\PM{\hs1 $\pm$ \hs1}
\def\np{\par\ni\hangindent=1.0 true cm\hangafter=1}
\def\up#1{\raise.8ex\hbox{\ssrm#1}}     \def\bsk#1{\baselineskip#1pt}
\def\sa{\rlap{$^{\ast}$}}               \def\"{\hs3\lower0.5ex\hbox{"}}
\def\sb{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'171}}}
\def\sc{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'172}}}
\def\sd{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'170}}}
\def\se{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'173}}}
\def\sf{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'153}}}
\def\sg{\rlap{\hs{0.4}$^{\ast\ast}$}}
\def\si{\rlap{\hs{0.4}\raise.7ex\hbox{\smdag\char'172\char'172}}}
\def\s#1{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm#1}}}
\def\sC{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm C}}}
\def\sG{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm G}}}
\def\sI{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm I}}}
\def\sN{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm N}}}
\def\sR{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm R}}}
\def\sT{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm T}}}
\def\sU{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm U}}}
\def\sW{\rlap{\hs{0.4}\raise.7ex\hbox{\ssrm W}}}
\def\ta{\llap{$^{\ast}$}\hs1}       
\def\tb{\llap{\raise.6ex\hbox{\smdag\char'171}}\hs1}
\def\tc{\llap{\raise.6ex\hbox{\smdag\char'172}}\hs1}
\def\td{\llap{\raise.6ex\hbox{\smdag\char'170}}\hs1}
\def\te{\llap{\raise.6ex\hbox{\smdag\char'173}}\hs1}
\def\tf{\llap{\raise.6ex\hbox{\smdag\char'153}}\hs1}
\def\tg{\llap{$^{\ast\ast}$}}
\def\ti{\llap{\raise.6ex\hbox{\smdag\char'172\char'172}}}
\def\t#1{\llap{\raise.7ex\hbox{\ssrm #1}}\hs0}
\def\tC{\llap{\raise.7ex\hbox{\ssrm C}}\hs1}
\def\tG{\llap{\raise.7ex\hbox{\ssrm G}}\hs1}
\def\tI{\llap{\raise.7ex\hbox{\ssrm I}}\hs1}
\def\tN{\llap{\raise.7ex\hbox{\ssrm N}}\hs1}
\def\tR{\llap{\raise.7ex\hbox{\ssrm R}}\hs1}
\def\tT{\llap{\raise.7ex\hbox{\ssrm T}}\hs1}
\def\tU{\llap{\raise.7ex\hbox{\ssrm U}}\hs1}
\def\tW{\llap{\raise.7ex\hbox{\ssrm W}}\hs1}
\def\thsp{\thinspace}    \def\msp{\kern.4em}     \def\sk{\hskip.6em\relax}
\def\kms{km~s$^{-1}$}    \def\kmss{km~s$^{-1}$\kern.25em}
\def\itkms{\hbox{{\it km s}\raise.6ex\hbox{\sit\hs{0.8}--\hs{0.5}1}}\hs1}
%\def\apjkms{\rm K{\srm M \hs1 S}$^{-1}$}
\def\asec{$''$}          \def\asecl{$''$\llap}   
\def\etal{{\it et al\/}.\hs3}       \def\setal{{\sit et al\/}.}
\def\etal#1{{\it et al\/}.\hs{-1.3}$^{#1}$}  
\def\b-v{($B-V$)}                   \def\u-b{($U-B$)}
\def\sec{\hbox{$''$\hskip-3pt .}}   \def\tsec{\hbox{$^s$\hskip-3pt .}}
\def\min{\hbox{$'$\hskip-3pt .}}    \def\tmin{\hbox{$^m$\hskip-3pt .}}
\def\Amm{\AA~mm$^{-1}$}             \def\Amms{\AA~mm$^{-1}$\kern .35em}
\def\msun{$M_{\odot}$\thsp}         \def\rsun{$R_{\odot}$\thsp}
\def\mbol{$M_{bol}$\thsp}           \def\mbs{$M_{bol \odot}$\thsp}
\def\degl{$^{\circ}$\hskip-1pt .}   \def\deg{\hbox{$^{\circ}$\hskip-3pt .}}
\def\dego{\raise.9ex\hbox{\smdag\char'16}}   \def\degs{\dego\hs3}
\def\hs#1{\hskip#1pt}               \def\hm#1{\hskip#1em} 
\def\frac#1/#2{\leavevmode\kern.05em\raise.6ex\hbox{\the\scriptfont0
    #1}\kern-.15em/\kern-.15em\lower.3ex\hbox{\the\scriptfont0 #2}}
\def\smfrac#1/#2{\leavevmode\kern.05em\raise.4ex\hbox{\the\scriptscriptfont0
    #1}\kern-.15em/\kern-.15em\lower.2ex\hbox{\the\scriptscriptfont0 #2}}
\def\itfrac#1/#2{\leavevmode\kern.05em\raise.6ex\hbox{\the\sit
    #1}\kern-.15em/\kern-.15em\lower.3ex\hbox{\the\sit #2}\hs1}
\def\itfracs#1/#2{\leavevmode\kern.05em\raise.6ex\hbox{\the\sit
    #1}\kern-.15em/\kern-.15em\lower.3ex\hbox{\the\sit #2}\hs4}
\def\corstop{\hbox{{\it C\hs{-1} oravel\/}.}\hs5}
\def\corcom{\hbox{{\it C\hs{-1} oravel\/},}\hs4}
\def\cor{\hbox{{\it C\hs{-1} oravel\/}}}      \def\cors{\cor\hs4}
\def\smcor{\hbox{\sit C\hs{-0.5}oravel\/}}    \def\smcors{\smcor\hs4}
\def\m{\hbox{\raise.8ex\hbox{\srm m}}}
\def\mag{\hbox{\raise.8ex\hbox{\srm m}\hskip-1pt .}}
\def\x{\hbox{\raise.2ex\hbox{,,}}}
\def\cont{(\hs{-1}{\it C\hs{-0.5}ontinued\/}\hs{0.5})}
\def\wt{wt.\hs{1.5}}

\hsize12truecm\hoffset2truecm\voffset2truecm\bsk{11}
\tabskip1.9em   \def\c{\hm{0.5}}
\brm\cl{\hm{-0.5}T{\rm ABLE} V}\ms\bit
\cl{\hm{-0.5}Radial-velocity observations of HD 17310            }
\vs4\it\cl{\hm{-1}The sources of the observations are as follows:}
\cl{2002--2004 --- published by Henry \etal9; 2005/2006 --- Cambridge \cor }
\bs\it
\hm{3.2}Date \hm{0.2}{\rm (}\hs{-1}UT\/{\rm )}\it\hm{3.8}MJD\hm{2.2}Velocity
\hm{1.0}Phase\hm{1.3}{\rm (}$O-C${\rm )\it\hm{1.5}`\hs1v\hs{1.5}sin\hs{1.5}i'}\vs1
\hm{16.4}\itkms\hm{5.6}\itkms\hm{1.8}\itkms
\rm\halign{\hm{-0.5}#\hfil\hm{-2.0}&\hfil#&\hfil#&    \hfil$#$\hm{0.2}&
\hm{-0.5}\hfil#\hm{0.2}&\hfil$#$&\hm1#\hfil\cr
\noalign{\filbreak\vs{12}}
 2002\hs4Sept.&25.411&  52542.411&   -3.7&$\overline{    39}$.104&   -2.9\cr
\noalign{\filbreak\vs{12}}
 2003\hs4Sept.&20.408&  52902.408&   -1.9&$\overline{    26}$.044&   -4.5\cr
\hskip2em 
     \hs4     &21.425&    903.425&   +1.1&.081&   +1.4\cr
\hskip2em 
     \hs4     &22.402&    904.402&   -3.7&.116&   -2.9\cr
\hskip2em 
     \hs4Oct. &28.379&    940.379&  +28.6&$\overline{    25}$.409&   +0.2\cr
\hskip2em 
     \hs4     &29.369&    941.369&  +28.6&.445&   -3.4\cr
\noalign{\filbreak\vs{12}}
 2004\hs4Sept.&25.427&  53273.427&  +29.7&$\overline{    13}$.381&   +4.4\cr
\hskip2em 
     \hs4     &26.385&    274.385&  +23.7&.416&   -5.4\cr
\hskip2em 
     \hs4     &27.371&    275.371&  +35.7&.451&   +3.1\cr
\hskip2em 
     \hs4     &28.344&    276.344&  +31.1&.486&   -4.8\cr
\hskip2em 
     \hs4     &29.370&    277.370&  +40.4&.523&   +1.4\cr
\noalign{\filbreak\vs{12}}
 2005\hs4Sept.&29.092&  53642.092&  +45.4&     0.633&   -0.3&\c9\cr
\hskip2em 
     \hs4Nov. &29.949&    703.949&  +37.0&     2.857&   -0.2&\c4.5\cr
\hskip2em 
     \hs4Dec. & 8.937&    712.937&   +2.9&     3.180&   +0.2&11\cr
\hskip2em 
     \hs4     &10.921&    714.921&   +9.5&.251&   -0.6&11\cr
\hskip2em 
     \hs4     &16.940&    720.940&  +32.4&.468&   -1.8&11.5\cr
\hskip2em 
     \hs4     &17.917&    721.917&  +40.4&.503&   +3.0&\c6.5\cr
\hskip2em 
     \hs4     &19.858&    723.858&  +44.3&.572&   +1.7&\c9\cr
\hskip2em 
     \hs4     &26.893&    730.893&  +40.1&.825&   -1.1&12.5\cr
\noalign{\filbreak\vs{12}}
 2006\hs4Jan. & 4.795&  53739.795&   +3.7&     4.145&   +3.4&\c9.5\cr
\hskip2em 
     \hs4     &25.836&    760.836&  +30.3&.902&   +0.8&\c8.5\cr
\hskip2em 
     \hs4     &28.814&    763.814&   +9.3&     5.009&   +1.6&13\cr
}
\bye

